Neural Graph Matching for Pre-training Graph Neural Networks

Recently, graph neural networks (GNNs) have been shown powerful capacity at modeling structural data. However, when adapted to downstream tasks, it usually requires abundant task-specific labeled data, which can be extremely scarce in practice. A promising solution to data scarcity is to pre-train a transferable and expressive GNN model on large amounts of unlabeled graphs or coarse-grained labeled graphs. Then the pre-trained GNN is fine-tuned on downstream datasets with task-specific fine-grained labels. In this paper, we present a novel Graph Matching based GNN Pre-Training framework, called GMPT. Focusing on a pair of graphs, we propose to learn structural correspondences between them via neural graph matching, consisting of both intra-graph message passing and inter-graph message passing. In this way, we can learn adaptive representations for a given graph when paired with different graphs, and both node- and graph-level characteristics are naturally considered in a single pre-training task. The proposed method can be applied to fully self-supervised pre-training and coarse-grained supervised pre-training. We further propose an approximate contrastive training strategy to significantly reduce time/memory consumption. Extensive experiments on multi-domain, out-of-distribution benchmarks have demonstrated the effectiveness of our approach. The code is available at: https://github.com/RUCAIBox/GMPT.

==> sec-def.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{asset/model.pdf}
    \caption{Overall framework of our proposed graph matching based GNN pre-training methods.}
    \label{fig:overall}
  \end{figure*}

\section{Preliminaries}\label{sec:prelim}

In this section, we  first introduce the task of graph supervised learning and present an overview of general GNN architecture~\cite{hamilton2017inductive}.

\paratitle{Graph supervised learning.} A graph can be represented as $G=(\mathcal{V},\mathcal{E}, \bm{X}, \bm{E})$,
where $\mathcal{V} = \{v_1, v_2, \ldots, v_{|\mathcal{V}|}\}$ denotes the node set,
$\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ denotes the edge set,
$\bm{X}\in \mathbb{R}^{|\mathcal{V}|\times d_{v}}$
and $\bm{E} \in \mathbb{R}^{|\mathcal{E}|\times d_{e}}$ represent the $d_v$- and $d_e$-dimensional attribute matrix for nodes and edges, respectively.
Furthermore, each graph is possibly associated with some label $y$ from a label set $\mathcal{Y}$. 
Given a set of graphs with labels $\{(G_1, y_1),(G_2, y_2), \ldots, (G_N, y_N)\}$,
the purpose of graph supervised learning is to learn graph representation embedding $\bm{h}_G$ for the entire graph $G$ and further utilize $\bm{h}_G$  to predict the corresponding label $y$.
By sampling a node (called \emph{central node}) and its neighborhood as a subgraph, 
tasks defined on the central node can be viewed as graph classification tasks,
\eg domain classification on citation networks~\cite{kipf2017semi,velickovic2018graph,lu2021learning}.
In this case, labels of the sampled subgraph are actually central node's labels.

\paratitle{Graph Neural Networks (GNNs).}
GNNs leverage graph structure as well as node and edge features
to learn a representation vector $\bm{h}_v$ for each node $v \in G$,
or the entire graph $\bm{h}_G$.
Modern GNNs adopt a neighborhood aggregation strategy.
Each node's representation is iteratively updated
by aggregating representations of its neighboring nodes and edges~\cite{hamilton2017inductive}.
After $k$ iterations of aggregation,
a node's representation captures its $k$-hop network neighborhood's structural features.
Formally, the $k$-th layer of a GNN can be summarized by the following expression:
\begin{align*}
    \bm{g}^{(k)}_v = & \operatorname{Aggregate}^{(k)}\left(\{\bm{h}^{(k-1)}_v,\bm{h}^{(k-1)}_u,\bm{e}^{(k-1)}_{uv}|u\in\mathcal{N}_v\}\right),\\
    \bm{h}^{(k)}_v = & \operatorname{Update}^{(k)}(\bm{h}^{(k-1)}_v,\bm{g}^{(k)}_v),
\end{align*}
where $\bm{h}^{(k)}_v$ is the representation of node $v$ at the $k$-th layer/iteration,
$\bm{e}_{uv}$ is the feature vector of edge between node $u$ and $v$, 
$\mathcal{N}_v$ is the set of nodes adjacent to node $v$, and 
$\bm{h}^{(0)}_v$ is initialized as node $v$'s node attributes $\bm{x}_v$.
To obtain the representation of the entire graph,
a permutation-invariant function $\operatorname{READOUT}$ pools node features after the last iteration $K$,
\begin{equation*}
    \bm{h}_G = \operatorname{READOUT}\left(\{\bm{h}_v^{(K)}|v\in G\}\right).\label{eq:gnn-readout}
\end{equation*}


In this work, we focus on pre-training GNNs: GNNs that are initialized with pre-trained parameters
are fine-tuned according to various downstream tasks.
Given the defined graph learning task, we consider two kinds of  GNN pre-training paradigms based on whether graph labels are used or not during pre-training: \emph{self-supervised setting} (without graph labels) and \emph{supervised setting} (with graph labels). %




